A Map of Bandits for E-commerce

The rich body of Bandit literature not only offers a diverse toolbox of algorithms, but also makes it hard for a practitioner to find the right solution to solve the problem at hand. Typical textbooks on Bandits focus on designing and analyzing algorithms, and surveys on applications often present a list of individual applications. While these are valuable resources, there exists a gap in mapping applications to appropriate Bandit algorithms. In this paper, we aim to reduce this gap with a structured map of Bandits to help practitioners navigate to find relevant and practical Bandit algorithms. Instead of providing a comprehensive overview, we focus on a small number of key decision points related to reward, action, and features, which often affect how Bandit algorithms are chosen in practice.

==> sections/ref_method.tex <==
%%\textcolor{red}{Pseudo-code side by side (as that in patent filing); Math discussion on the difference between general RL and Bandit}

%In a sequential content recommendation, the impact of ‘sequential’ occurs in two directions: an early impression may affect the success probability of a later impression (forward) and a reward can be attributed to not just the immediate last impression but earlier impressions (backward). 

%Traditionally, Multi-Armed Bandit (MAB) methods have been frequently used for the content optimization use cases. To model the forward effects, we added the content on the prior page as the feature of the bandit on the next page. To capture the backward effects, we utilize the long-term reward, which is defined as the final outcome of the customers after viewing the flow, as the objective of the bandits. 

%In a multi-page sequential content recommendation, the impact of `sequential' occurs in two directions: an early impression may affect the success probability of a later impression (forward) and a reward can be attributed to not just the short-term last impression but earlier impressions (backward). 

\subsection{Problem Formulation}
We model sequential decision making in linear flow as a MDP. Let $D$ be number of the pages that content recommendation is needed. For each page $i$, there are $N_{i}$ content candidates that we can choose from. The selected content can be denoted as $a_{i,n_i}$ where $n_i \in \{ 1, 2, \cdots, N_{i} \}$. For simplicity, we will denote the content shown on page $i$ as $a_{i}$ unless the notation $a_{i,n_i}$ is needed to distinguish between different content for page $i$. The flow starts with state $S_{1, X}$ where $X$ is customer feature vector. After action $a_{i}$ is selected to show to customer with features $X$ on page $i$, there are two possible states: $S_{i+1, X, a_{i}}$ and $S_{Exit}$. The only exception is for the last page, page $D$, the two possible states after action $a_{D}$ are: $S_{End}$ and $S_{Exit}$. $S_{i+1, X, a_{i}}$ means customers move forward in the process to the next page after seeing $a_{i}$. $S_{Exit}$ means customers drop from the process without reaching the end and $S_{End}$ means customers reached the end. We denote $R_{i}$ and $G_{i}$ as short--term and long--term rewards after action ${a_{i}}$ respectively. The goal from a linear flow is to optimize $G_1$.

% \begin{figure*}
%   \includegraphics[width=0.8\textwidth]{MDP.png}
%   \caption{Illustration of the Linear-flow MDP}
%   \label{fig:mdp}
% \end{figure*}

In Prime cancellation use case, $D$ is $3$ and $a_{i}$ are marketing content designed to retain customers. Customers are at $S_{1, X}$ after they click on the End Membership button. We may have Prime benefits usage and tenure features in $X$. We may also include the upstream channel that customers landed from in $X$. Customers get to $S_{Exit}$ if they drop from the cancellation process at any page leading to $R_{i} = 1$. Customers are in $S_{i+1, X, a_{i}}$ if they move on in the process after marketing content $a_{i}$. The short-term reward is 0 from entering $S_{i+1, X, a_{i}}$. $S_{End}$ is another termination state other than $S_{Exit}$. Customers reach this state if they cancel their membership after seeing content on the last page. This leads to $R_{D} = 0$.  

\subsection{Transition Probability Matrix Modeling}
We use contextual Bandit to model and update transition probability matrix. As our reward are binary and there can be only two outcomes per action, we use Bayesian linear Probit regression \cite{BLIP} to model our reward. The transition probability is formulated through a Probit link function. After showing page $i$, the probability of customers moving forward in the process and dropping from the process is formulated as in Equations \ref{eq:1} and \ref{eq:2} respectively. By using this formulation, we model only interdependence between two successive pages. For page 1, $a_{i-1}$ is dropped from the subscripts but the rest of the equations remain the same.

\begin{equation}
P(S_{t+1} = S_{i+1, X, a_{i}}|S_{t} = S_{i, X, a_{i-1}}, a_{t} = a_{i}) = \Phi(-1 * \frac{B_{X, a_{i-1}, a_{i}}^TW_{i}}{\beta}) \label{eq:1}
\end{equation}


\begin{equation}
P(S_{t+1} = S_{Exit}|S_{t} = S_{i, X, a_{i-1}}, a_{t} = a_{i}) = \Phi(\frac{B_{X, a_{i-1}, a_{i}}^TW_{i}}{\beta}) \label{eq:2}
\end{equation}

In the formula, $\Phi$ is cumulative distribution function for standard normal distribution. $\beta$ is a scaling hyperparameter. $W_{i}$ are the weights quantifying feature contributions to the utility function. $B_{X, a_{i-1}, a_{i}}$ is the final vector that we will learn weights for and formed by combining $X$, $a_{i-1}$ and $a_{i}$ (usually with interaction terms). $B_{X, a_{i-1}, a_{i}}$ is the reason why we can easily model content incompatibility. To explain this, let's first assume we have one feature $x$ for $X$, $a_{i-1}$ has two candidates: $a_{i-1,1}$ and $a_{i-1,2}$, and $a_{i}$ has three candidates: $a_{i,1}$, $a_{i,2}$ and $a_{i,3}$. We know $a_{i,3}$ cannot be shown if $a_{i-1,1}$ is shown to customers. We may set $B_{a_{i-1}, a_{i}}$ as in Equation \ref{eq:3} where we have $1$ for intercept and contextual feature interacting with action terms. We recognize content incompability between $a_{i-1,1}$ and $a_{i,3}$ by simply omitting interaction term $x \cdot a_{i-1,1} \cdot a_{i,3}$ in the equation. In addition, we can interpret interdependence strength between pages by checking the weights for the interaction terms across pages.

% \begin{equation}
% 	\begin{split}
% 		B_{X, a_{i-1}, a_{i}}^T &= (1, x \cdot a_{i,1}, x \cdot a_{i,2}, x \cdot a_{i,3}, \\
% 		&x \cdot a_{i-1,1} \cdot a_{i,1}, x \cdot a_{i-1,1} \cdot a_{i,2}, \\
% 		&x \cdot a_{i-1,2} \cdot a_{i,1}, x \cdot a_{i-1,2} \cdot a_{i,2}, x \cdot a_{i-1,2} \cdot a_{i,3}) \label{eq:3} \\
% 	\end{split}
% \end{equation}

\begin{equation}
  \begin{split}
    B_{X, a_{i-1}, a_{i}}^T &= (1, x \cdot a_{i,1}, x \cdot a_{i,2}, x \cdot a_{i,3}, \\
    &a_{i-1,1} \cdot a_{i,1}, a_{i-1,1} \cdot a_{i,2}, \\
    &a_{i-1,2} \cdot a_{i,1}, a_{i-1,2} \cdot a_{i,2}, a_{i-1,2} \cdot a_{i,3}) \label{eq:3} \\
  \end{split}
\end{equation}

We assume the weights $W_{i}$ follow Normal distribution parameterized by a mean vector $\boldsymbol{\mu}_{W_i}$ and variance vector $\boldsymbol{\nu}_{W_i}$. We update the distribution from prior to posteriror by enforcing Normal distribution as the distribution type and obtaining the distribution parameters by minimizing KL-divergence from the approximate normal distribution and the exact distribution \cite{BLIP}.  

\subsection{RL Policy and Policy Updating}
We propose Algorithm \ref{alg:seqTS} \textit{MDP with Bandits} to solve the formulated MDP. $\mathscr{D}_d$ denotes the dataset for updating contextual Bandit for Page $d$. $k$ denotes the $k^{th}$ impression. $a_i^*(a_{i-1})$ denotes the optimal action for page $i$ given content on page $i-1$. The complexity of the algorithm is $O(DN^2K)$ assuming number of content on each page is $N$ for discussion simplicity. For each observation, we sample weights from their posterior distribution using TS for calculating transition probability matrix. We then employ exact DP to allocate the optimal series of content to show on each page given the weights. Per reward signal availability, we update the weights distributions and the loop repeats. If we get the feedback signal in batches, the algorithm alters on Lines 11 and 12 where we would have the updates at batch level instead of observation level.

\begin{algorithm}
\begin{algorithmic}[1]
\State Init $\mathscr{D}_1 = \mathscr{D}_2 = \cdots = \mathscr{D}_D = \oldemptyset$
\For{$k = 1,\cdots, K$}
    \State Receive context $x_k$ and Initiate $\E[G|a_D] = 0$
    \State Sample $W_{1}, \cdots, W_{D}$ from the posterior $P(W_1|\mathscr{D}_1),\cdots, P(W_D|\mathscr{D}_D)$ \algorithmiccomment{TS}
    \For{$i = D, D - 1, \cdots, 2$} \algorithmiccomment{Line 5 - 9: Exact DP}
        \For{ $a_{i - 1}$ in content pool of page $i - 1$}: 
            \begin{gather}    \label{eq:eq2}
            \begin{split}
                a_i^*(a_{i-1}) = \underset{a_{i}}{\argmax} \big\{ \E[R|a_{i}, a_{i-1}, x_k; W_{i}] +& \\
                (1 - \E[R|a_{i}, a_{i-1}, x_k; W_{i}]) * \E[G|a_{i}] \big\}&
            \end{split}
            \end{gather}
            \begin{gather}    \label{eq:eq3}
            \begin{split}
                \E[G|a_{i - 1}] = \E[R|a_i^*(a_{i-1}), a_{i-1}, x_k; W_{i}] + &\\
                (1 - \E[R|a_i^*(a_{i-1}), a_{i-1}, x_k; W_{i}]) * \E[G|a_{i}]&
            \end{split}
            \end{gather}
        \EndFor
    \EndFor
\State $a_1^* = \underset{a_{1}}{\argmax} \big\{ \E[R|a_{1}, x_k; W_1] + (1-E[R|a_{1}, x_k; W_1])\E[G|a_{1}]\big\} $
\State Display layout $\{a_1^*,a_2^*(a_1^*),\cdots, a_{D}^*(a_{D-1}^*)\}$ and observe reward $R_{1,k}, \cdots, R_{D,k}$
\State Update $\mathscr{D}_1 = \mathscr{D}_1 \cup (x_{k}, a_{1k}, R_{1k})$ and Update $\boldsymbol{\mu}_{W_1}$, $\boldsymbol{\nu}_{W_1}$ \algorithmiccomment{BLIP Updating \cite{BLIP}}
\State Update $\mathscr{D}_i = \mathscr{D}_i \cup (x_{k}, a_{ik}, a_{i-1,k}, R_{i,k})$ and Update $\boldsymbol{\mu}_{W_i}$, $\boldsymbol{\nu}_{W_i}$ for $i\in \{2,3,\cdots,D\}$ if $a_{ik}$ was presented
\EndFor
\end{algorithmic}
%\caption{MDP solved with Contextual Bandit, Thompson Sampling and Exact Dynamic Programming}
\caption{MDP with Bandits}
\label{alg:seqTS}
\end{algorithm}

% %%% From before
% In this section, we introduce three methods to solve the sequential recommendation problem: bandit methods, Q-learning with $\epsilon$-greedy, and bandit with sequantial TS. In our bandit methods, we propose several models with variations of modeling reward and construct features. In each page, we make decisions independently according to the model of this page. In the bandit with sequential TS, we leverage bandits to model the short-term reward in each page, and then apply sequential TS to make decisions on all the pages at the same time.

% \subsection{Bandit Methods}

% Traditionally, MAB methods have been frequently used for the 1-page content optimization. We leverage MAB as our benchmark solution. We build an independent bandit model for each of the pages and recommend the content on each of the pages purely based on the bandit model of the according page.

% \subsubsection{Model Training}

% We BLIP \cite{BLIP} to model the reward of each page:

% \begin{equation}
% P(R|B_{A, X}) = \Phi(R * \frac{B_{A,X}^TW}{\beta}) \label{eq:1}
% \end{equation}

% where $R$ is the binary reward function, $A$ is the content of each page, $X$ is the features, $B$ is the vector that combines customer features $X$ and content candidates $A$, $\Phi$ is the probit function, $\beta$ is a scaling hyperparameter. The goal is to learn the model parameters $W$.

% There are mainly 3 dimensions of variations in modeling this problem:

% \begin{enumerate}
% \item Short-term reward vs. Long-term reward: whether use short-term reward $R_i$ or long-term reward $G_i$ as the reward function for the model of page $i$.
% \item Independence vs. One-Step Dependence: Whether we assume the behaviors of each page are independent. If not, we utilize the content of last page as the feature in the next page's model (one-step dependent). 
% \item Interaction between features and arms vs. no Interaction: if we assume one-step dependent, whether the effects of a content on the last page are the same for all the arms at this page.
% \end{enumerate}

%  To simplify the notation, we use $R \sim A$ to represent the model with $R$ as the reward and $A$ as the arm; $R \sim A + X$ to represent the BLIP model with $R$ as the reward, $A$ as the arm and $X$ as the feature. Sometimes we also add the (arm, feature) interaction terms which is denoted as $X:A$. We summarize the models of the 6 treatments in the table \ref{table:banditReg}. In the description column, we use short, long, Ind, Dep, Inter to represent short-term reward, long-term reward, Independence, One-Step Dependence and Interaction respectively.

% % \begin{figure}
% %   \centering
% %   \includegraphics[width=\textwidth]{banditTreatments.png}
% %   \caption{Bandit Treatments}
% %   \label{fig:banditTreatments}
% % \end{figure}

% \begin{table}[h]
% \centering
% \caption{Bandit Treatments Regression}
% \label{table:banditReg}
% \begin{tabular}{|l|l|l|}
% \hline
% Treatment & Description & Linear Term \\
% \hline
% $T_{S,I}$ & Short, Ind & Page 1: $R_1 \sim a_1$; Page $i$: $R_i \sim a_i$ for $i\in 2,\cdots,D$ \\ 
% \hline
% $T_{S,D}$ & Short, Dep& Page 1: $R_1 \sim a_1$; Page $i$: $R_i \sim a_i + a_{i - 1}$ \\ 
% \hline
% $T_{S,D,I}$ & Short, Dep, Inter& Page 1: $R_1 \sim a_1$; Page $i$: $R_i \sim a_i + a_{i - 1} + a_{i - 1}:a_i$  \\ 
% \hline
% $T_{L,I}$ & Long, Ind& Page 1: $G_1 \sim a_1$; Page $i$: $G_i \sim a_i$ \\ 
% \hline
% $T_{L,D}$ & Long, Dep& Page 1: $G_1 \sim a_1$; Page $i$: $G_i \sim a_i + a_{i - 1}$ \\ 
% \hline
% $T_{L,D,I}$ & Long, Dep, Inter& Page 1: $G_1 \sim a_1$; Page $i$: $G_i \sim a_i + a_{i - 1} + a_{i - 1}:a_i$  \\ 
% \hline
% \end{tabular}
% \end{table}

% In the appendix \ref{compareBanditTreatments}, we compare the treatments above and conclude that treatments $T_{L,I}, T_{L,D}, T_{L,D,I}$ are expected to outperform other treatments.

% \subsubsection{Online Recommendation}

% We model $W$ in the formula \eqref{eq:1} as mutually independent random variable following a Gaussian posterior distributions, with Bayesian updates over an initial Gaussian prior of $\mathcal{N}(0,1)$. We update $W$ using observations based on formula (7) and (8) in the paper Graepel et al 2010 \cite{BLIP} and then pull arms based on Thompson Sampling \cite{TS, TSContextual}.

% \subsection{Q-Learning}

% Reinforcement Learning is a nature method to model this problem. We leverage a classic model-free algorithm Q-Learning to learn the value function of (state, action) pair and then use $\epsilon$-greedy as the online policy. It estimates the value function offline based on Bellman equation:
% \begin{equation}
% Q(s_t, a_t) \leftarrow Q(s_t, a_t) + \alpha * (r_t + \gamma * \max_{a} Q(s_{t+1}, a) - Q(s_t, a_t))
% \end{equation}
% Where $\alpha$ is the learning rate, $\gamma$ is the discount factor (it is 1 in our use case), $r_t$ is the short-term reward. We use $\epsilon$-greedy as the online policy: play the best action with $1 - \epsilon$ probability and randomly play any action with $\epsilon$ probability.

% \subsection{Bandit with Sequential Thompson Sampling}

% In the Bandit methods, it leverages bandit to model the performance and make action at each page separately. However, as the online recommendation of each page is independent, the result is likely to be local optimal. To provide global optimization solution, we propose a new policy called Sequential Thompson Sampling (SeqTS). We still leverage BLIP to model the short-term reward and pull the best combination after sampling the reward distributions based on SeqTS described in Algorithm \ref{alg:seqTS}. We use model $T_{S, D}$ and $T_{S,D,I}$ in the Table \ref{table:banditReg} to model the short-term reward function without interaction terms and with interaction terms respectively (treatments are annotated as $T_{SeqTS}, T_{SeqTS, I}$).

% \begin{algorithm}
% \begin{algorithmic}[1]
% \State Init $\mathscr{D}_1 = \mathscr{D}_2 = \cdots = \mathscr{D}_D = \oldemptyset$
% \For{$t = 1,\cdots, T$}
%     \State Receive context $x_t$ and Initiate $\E[G|a_D] = 0$
%     \State Sample $w_{1}, \cdots, w_{D}$ from the posterior $P(w_1|\mathscr{D}_1),\cdots, P(w_D|\mathscr{D}_D)$ \algorithmiccomment{Similar to TS}
%     \For{$i = D, D - 1, \cdots, 2$} \algorithmiccomment{Find best combination based on Dynamic Programming}
%         \For{ $a_{i - 1}$ in content pool of page $i - 1$}: 
%             \begin{gather}    \label{eq:eq2}
%                 a_i^*(a_{i-1}) = \underset{a_{i}}{\argmax} \E[R|a_{i}, a_{i-1}, x_t; w_{i}] + (1 - \E[R|a_{i}, a_{i-1}, x_t; w_{i}]) * \E[G|a_{i}] 
%             \end{gather}
%             \begin{gather}    \label{eq:eq3}
%                 \E[G|a_{i - 1}] = \E[R|a_i^*(a_{i-1}), a_{i-1}, x_t] + (1 - \E[R|a_i^*(a_{i-1}), a_{i-1}, x_t]) * \E[G|a_{i}] 
%             \end{gather}
%         \EndFor
%     \EndFor
% \State $a_1^* = \underset{a_{1}}{\argmax} \E[R|a_{1}, a_{0}, x_t; w_{1}] + \E[G|a_{1}]$
% \State Display layout $\{a_1^*,a_2^*(a_1^*),\cdots, a_{D}^*(a_{D-1}^*)\}$ and observe reward $R_{1,t}, \cdots, R_{D,t}$
% \State Update $\mathscr{D}_1 = \mathscr{D}_1 \cup (x_{t}, a_{1t}, R_{1t})$
% \State Update $\mathscr{D}_i = \mathscr{D}_i \cup (x_{t}, a_{it}, a_{i-1,t}, R_{i,t})$ for $i\in \{2,3,\cdots,D\}$
% \EndFor
% \end{algorithmic}
% \caption{Sequential Thompson Sampling (SeqTS)}
% \label{alg:seqTS}
% \end{algorithm}

% The complexity of SeqTS is $O(DNT)$, where $D, N, T$ is number of pages, number of contents on each page, and number of rounds respectively. In the equation \eqref{eq:eq2} \eqref{eq:eq3}, we maximize the long-term reward defined in the equation \eqref{eq:eq0} based on dynamic programming.

% Our algorithm is most similar to Posterior Sampling for Reinforcement Learning (PSRL), a Bayesian-based Reinforcement learning model described in the paper Osband et al 2013 \cite{PSRL}. But our algorithm has the advantages: \textbf{1)} It does not require building a new RL system which requires heavy engineering effort. And for the teams who have already onboarded Bandit, the onboarding effort to SeqTS is very light. \textbf{2)} In the PSRL, each (state, action) pair is modeled separately in terms of distributions like Dirichlet. In the Bandit with SeqTS, we model all the (state, action) pairs of a state using one Bayesian Bandit like BLIP. \textbf{3)} SeqTS directly gives the analytical best action combination. In PSRL, it relys on Policy Evaluation to solve the MDP and return the best action at each state. Therefore, SeqTS has much lower complexity. 

% More detailed comparison of Bandit with SeqTS and PSRL is in the appendix \ref{STS}.






==> sections/ref_table.tex <==
Using simulation, we compare the proposed \textit{MDP with Bandits} algorithm to three other algorithms: independent Bandits, interaction Bandits and Q-learning. Independent Bandits algorithm assumes no interdependence across pages. TS for each Bandit model is conducted separately for each page. Interaction Bandits algorithm models interdependence in two succesive pages by using the content shown in a previous page to construct features in the Bandit formulation. Other than the feature construction, TS for each Bandit model in the interaction Bandits algorithm is also conducted separately. As shown in Table \ref{table:alg_set}, in MDP with Bandits, we use short-term reward $R_i$ as the feedback signal for Bandits while independent and interaction Bandits use the long-term reward $G_i$ as the feedback signal. For notation simplicity, we use the tide sign $\sim$ to introduce the linear model form used for Equations \ref{eq:1} and \ref{eq:2} with Probit link function assumed as default. The Bandits forms only involve content features to highlight the action interaction. MDP with Bandits and interaction Bandits have the same linear model form. Lift in performance from MDP with Bandits (if any) directly quantifies the benefit of modeling the process as a MDP instead of a series of Bandits. For Q-learning, we follow the vanilla setup: we model the content shown in the previous page as the state and update the Q-Table based on Bellman Equation. We set the learning rate to be 0.05 and discount factor to be 1. The policy is based on $\epsilon\-$greedy with $\epsilon$ linearly decreases from 0.05 (2nd batch) to 0.01 (last batch).

% \begin{table*}[h]
% \centering
% \caption{Algorithms in Comparison}
% \label{table:alg_set}
% \begin{tabular}{|l|l|l|}
% \hline
% Algorithm & Linear model form & \# parameters \\
% \hline
% MDP with Bandits &  Page 1: $R_1 \sim a_1$; Page $i$: $R_i \sim a_i + a_{i - 1} + a_{i - 1}:a_i$ for $i\in 2,\cdots,D$  & $O(DN^2)$ \\ 
% \hline
% Interaction Bandits & Page 1: $G_1 \sim a_1$; Page $i$: $G_i \sim a_i + a_{i - 1} + a_{i - 1}:a_i$ & $O(DN^2)$ \\ 
% \hline
% Independent Bandit & Page 1: $G_1 \sim a_1$; Page $i$: $G_i \sim a_i$ & $O(DN)$\\ 
% \hline
% \end{tabular}
% \end{table*}

\begin{table*}[h]
\centering
\caption{Algorithms in Comparison}
\label{table:alg_set}
\begin{tabularx}{{X|l}}
\textbf{Algorithm} & \textbf{Linear model form} & \textbf{Parameters}\\
\hline
MDP with Bandits &  Page 1: $R_1 \sim a_1$; Page $i$: $R_i \sim a_i + a_{i - 1} + a_{i - 1}:a_i$ for $i\in 2,\cdots,D$  & $O(DN^2)$ \\ 
Interaction Bandits & Page 1: $G_1 \sim a_1$; Page $i$: $G_i \sim a_i + a_{i - 1} + a_{i - 1}:a_i$ & $O(DN^2)$ \\ 
Independent Bandit & Page 1: $G_1 \sim a_1$; Page $i$: $G_i \sim a_i$ & $O(DN)$\\ 
\end{tabularx}
\end{table*}


\subsection{Simulated Data}
We generate simulation data assuming Probit link function between short-term reward $R_{i}$ and $B_{X, a_{i-1}, a_{i}}^TW_{i}$ based on equations \ref{eq:1} and \ref{eq:2}, with $\beta$ set as $1 + \alpha_1 + \alpha_c + \alpha_2$ and the linear model forms for $B_{X, a_{i-1}, a_{i}}^TW_{i}$ specified as in equation \ref{eq:sim_first} for first page and equation \ref{eq:sim} for the other pages. Similar to \cite{MVT}, we use the $\alpha_1$, $\alpha_c$ and $\alpha_2$ to separately control the importance of content to recommend on the current page, content already shown on the previus page, and the interaction between them. For each simulation run, the ground truth weights $W_i$ are sampled independently from a normal distribution with mean $0$ and variance $1$ except for $w_i^0$. Mean for $w_i^0$ is set as $\Phi^{-1}(x)\beta$ where $x$ reflects the average success rate. With a larger value for $\alpha_2$, interdependence across pages is set stronger.

\begin{equation}
B_{X, a_{1}}^TW_{1} = w^0_1 + \alpha_1 \sum_{n_1=1}^{N_1} w_{n_1}^1 a_{1,n_1} + \alpha_1 \sum_{x} w_{x}^1 x \label{eq:sim_first}
\end{equation}

\begin{equation}
	\begin{split}
		B_{X, a_{i-1}, a_{i}}^TW_{i} &= w^0_i + \alpha_1 \sum_{n_i=1}^{N_i} w_{n_i}^1 a_{i,n_i} + \alpha_1 \sum_{x} w_{x}^1 x + \\
    &\alpha_c \sum_{n_{i-1}=1}^{N_{i-1}} w_{n_{i-1}}^c a_{i-1,n_{i-1}} + \\
    &\alpha_2 \sum_{n_i=1}^{N_i} \sum_{n_{i-1}=1}^{N_{i-1}} w_{n_i,n_{i-1}}^2 a_{i,n_i} a_{i-1,n_{i-1}} + \\
    &\alpha_2 \sum_{n_i=1}^{N_i} \sum_{x} w_{n_i,x}^2 a_{i,n_i} x \quad \textrm{for} \quad  i\in 2,\cdots,D \label{eq:sim} \\
	\end{split}
\end{equation}

For each simulation, we sample the actual weights in equations \ref{eq:sim_first} and \ref{eq:sim} once and we calculate the long-term reward of each combination $(a_1, \cdots, a_D)$ as:

\begin{equation}
\E[G|W,a_1,\cdots,a_D] = \E[R_1 + (1 - R_1)R_2 + \cdots + \Pi_{i=1}^{D-1}(1 - R_i)R_D] \label{eq:expected_reward}
\end{equation} 
where $R_i = \Phi(\frac{B_{X,a_{i-1}, a_{i}}^TW_{i}}{\beta}) \quad \textrm{for} \quad  i\in 2,\cdots,D$ and $R_1 = \Phi(\frac{B_{X, a_{1}}^TW_{1}}{\beta})$. 

The series of actions for each algorithm are selected by itself. Given sampled weights and selected actions, empirical rewards ($R$) are sampled from the data generation model. Actual reward $G_k$ is 0 if any $R_k$ is 0. Each simulation was run for $K = 14k$ time steps with updating batch size $1k$ to mimic a 2 week experiment. We ran $100$ simulations and report the averaged performance of each algorithm using batch size normalized cumulative regret:
\begin{equation}
\frac{1}{\# runs}\sum_{j=1}^{\# runs} \frac{1}{batchSize}\sum_{k = 1}^{K} (\E[G|W,a_{1,j}^*, \cdots, a_{D,j}^*] - G_{j,k}) \label{eq:regret}
\end{equation} 

Where $\E[G|W,a_{1,j}^*, \cdots, a_{D,j}^*]$ is the best expected long-term reward for $j^{th}$ run and $G_{j,k}$ is the long-term reward for $i^{th}$ run and $k^{th}$ time step.

\subsection{Simulation Results}

\begin{figure}[tb]
\centering
\begin{minipage}[b]{.48\textwidth}
  \centering
  \includegraphics[width=1.0\textwidth]{darwinStrength=2.png}
  \caption{Example run of algorithms on simulated data with $\alpha_1=1, \alpha_c=1, \alpha_2=2$~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~}
  \label{fig:darwinStrength2}
\end{minipage}%
\hfill
\begin{minipage}[b]{.48\textwidth}
  \centering
  \includegraphics[width=1.0\textwidth]{darwinContext.png}
  \caption{Example run of algorithms on simulated data with $\alpha_1=1, \alpha_c=1, \alpha_2=2$ and 1 categorical feature with 3 categories}
  \label{fig:darwinContext}
\end{minipage}
\end{figure}

\begin{figure}[tb]
\centering
\begin{minipage}[b]{.48\textwidth}
  \centering
  \includegraphics[width=1.0\textwidth]{darwinPage.png}
  \caption{Algorithm performance as number of pages vary. $\alpha_1 = 1, \alpha_2 = 1, \alpha_2 = 2$}
  \label{fig:darwinPage}
\end{minipage}%
\hfill
\begin{minipage}[b]{.48\textwidth}
  \centering
    \includegraphics[width=1.0\textwidth]{darwinStrength.png}
  \caption{Algorithm performance as $\alpha_2$ is varied. $\alpha_1=1, \alpha_c=1$}
  \label{fig:darwinStrength}
\end{minipage}
\end{figure}

We first compare the performance with $\alpha_1=1, \alpha_c=1, \alpha_2=2$ in both non-contextul and contextual use case. In the contextual case, we include $14$ categorical feature with $3$ equally-likely categories. We assume $3$ pages and each page has $3$ content candidates. Results are shown in figures \ref{fig:darwinStrength2} and \ref{fig:darwinContext}. The proposed algorithm converges faster than all the other three. Also, it has the lowest cumulative regret followed by interaction Bandits. This means when there is considerable interdependence across pages, modeling interactions in the transition probability reduces regrets and modeling the process as a MDP instead of separate Bandits further lifts the performance. On the other hand, bandit algorithms with TS generally outperform Q\-learning with $\epsilon$-greedy, given its efficiency in exploration.

We then take a look at the impact of number of pages on performance, shown in figure \ref{fig:darwinPage}. The number of pages varies from $2$ to $6$ and that of content combinations $N^D$ varies from $9$ to $729$. MDP with Bandits consistently outperforms the other three algorithms. The performance advantage over Q-learning shrinks with increasing page number. 


To test the model's sensitivity to interdependence strength, we conduct a set of simulation runs with $\alpha_2$ increasing from 0 to 3 while fixing $\alpha_1$ and $\alpha_c$ at $1$. Results are shown in figure \ref{fig:darwinStrength}. When $\alpha_2$ is $0$, independent bandits algorithm outperforms the other two bandit algorithms as both interaction Bandits and MDP with Bandits require traffic to learn the weights for interaction terms should actually be set as $0$. As $\alpha_2$ increases, MDP with Bandits starts to outperform. As Q-learning directly learns the Q function by Bellman equation, interaction strength has minor influence to its performance. Overall, the performance for MDP with Bandits is consistently better than all other algorithms when interaction strength is greater than 1.


